Mitigating Spurious Correlations for Self-supervised Recommendation

Recent years have witnessed the great success of self-supervised learning (SSL) in recommendation systems. However, SSL recommender models are likely to suffer from spurious correlations, leading to poor generalization. To mitigate spurious correlations, existing work usually pursues ID-based SSL recommendation or utilizes feature engineering to identify spurious features. Nevertheless, ID-based SSL approaches sacrifice the positive impact of invariant features, while feature engineering methods require high-cost human labeling. To address the problems, we aim to automatically mitigate the effect of spurious correlations. This objective requires to 1) automatically mask spurious features without supervision, and 2) block the negative effect transmission from spurious features to other features during SSL. To handle the two challenges, we propose an invariant feature learning framework, which first divides user-item interactions into multiple environments with distribution shifts and then learns a feature mask mechanism to capture invariant features across environments. Based on the mask mechanism, we can remove the spurious features for robust predictions and block the negative effect transmission via mask-guided feature augmentation. Extensive experiments on two datasets demonstrate the effectiveness of the proposed framework in mitigating spurious correlations and improving the generalization abilities of SSL models. The code is available at https://github.com/Linxyhaha/IFL.

==> mir-sample-bib.tex <==
\begin{thebibliography}{9}



\bibitem{bib1} B. Ran, D. E. Boyce. {\sl Modeling Dynamic Transportation Network}, Berlin, Germany: Springer-Verlag, pp. 69-83,1996. (Book style)

\bibitem{bib2} G. O. Young. Synthetic structure of industrial plastics. Plastics, 2nd ed., J. Peters, Ed., New York, USA: McGraw-Hill, pp. 15-64, 1964. (Book style with paper title and editor)

\bibitem{bib3} L. C. Su, F. Zhu. Design of a novel omnidrectional stereo vision system. {\sl Acta Automatica Sinica}, vol. 32, no. 1, pp. 67-72, 2006. (in Chinese) (Periodical style)

\bibitem{bib4} R. Roychoudhury, S. Bandyopadhyay, K. Paul. Adistributed mechanism for topology discovery in ad hoc wireless networks using mobile agents. In {\sl Proceedings of IEEE First Annual Workshop on Mobile and Ad hoc Networking and Computing}, IEEE, Piscataway, USA, pp. 145-146,2000. (Published Conference Proceedings style)

\bibitem{bib5} O. Hryniewicz. An evaluation of the reliability of complex systems using shadowed sets and fuzzy lifetime data. {\sl International Journal of Automation and Computing}, to be published.

\bibitem{bib6} W. Zhang. Reinforcement Learning for Job-shop Scheduling, Ph. D. dissertation, Oregon State University, USA,1996. (Dissertation style)

\bibitem{bib7} IEEE Criteria for Class IE Electric Systems, IEEE Standard 308, 1969. (Standards style)

\bibitem{bib8} R. C. Reily, J. L. Mack. The Self-organization of Spatially Invariant Representations, Technical Report PDP. CNS.92.5, Department of Psychology, Mellon University, USA, 1993. (Report style)

\bibitem{bib9} J. P. Wilkinson. Nonlinear Resonant Circuit Devices, U.S. Patent 362412, July 1990. (Patent style)

\bibitem{bib10} J. Jones. {\sl Networks}, 2nd ed., [Online], Available: http://www.atm.com, May 10, 1991.

\bibitem{bib11} R. J. Vidmar. On the use of atmospheric plasmas as electromagnetic reflectors. {\sl IEEE Transactions on Plasma Science}, vol. 21, no. 3, pp. 945-999, [Online], Available: http://www.halcyon.com, July 20-25, 1999.





\end{thebibliography}


